Benchmarking and Dissecting the Nvidia Hopper GPU Architecture

Graphics processing units (GPUs) are continually evolving to cater to the computational demands of contemporary general-purpose workloads, particularly those driven by artificial intelligence (AI) utilizing deep learning techniques. A substantial body of studies have been dedicated to dissecting the microarchitectural metrics characterizing diverse GPU generations, which helps researchers understand the hardware details and leverage them to optimize the GPU programs. However, the latest Hopper GPUs present a set of novel attributes, including new tensor cores supporting FP8, DPX, and distributed shared memory. Their details still remain mysterious in terms of performance and operational characteristics. In this research, we propose an extensive benchmarking study focused on the Hopper GPU. The objective is to unveil its microarchitectural intricacies through an examination of the new instruction-set architecture (ISA) of Nvidia GPUs and the utilization of new CUDA APIs. Our approach involves two main aspects. Firstly, we conduct conventional latency and throughput comparison benchmarks across the three most recent GPU architectures, namely Hopper, Ada, and Ampere. Secondly, we delve into a comprehensive discussion and benchmarking of the latest Hopper features, encompassing the Hopper DPX dynamic programming (DP) instruction set, distributed shared memory, and the availability of FP8 tensor cores. The microbenchmarking results we present offer a deeper understanding of the novel GPU AI function units and programming features introduced by the Hopper architecture. This newfound understanding is expected to greatly facilitate software optimization and modeling efforts for GPU architectures. To the best of our knowledge, this study makes the first attempt to demystify the tensor core performance and programming instruction sets unique to Hopper GPUs.

==> tex/background.tex <==
\section{Background}
New fourth-generation Tensor Cores are up to 6x faster chip-to-chip compared to A100, including per-SM speedup, additional SM count, and higher clocks of H100. On a per SM basis, the Tensor Cores deliver 2x the MMA (Matrix Multiply-Accumulate) computational rates of the A100 SM on equivalent data types, and 4x the rate of A100 using the new FP8 data type, compared to previous generation 16-bit floating-point options. The Sparsity feature exploits fine-grained structured sparsity in deep learning networks, doubling the performance of standard Tensor Core operations

New DPX Instructions accelerate dynamic programming algorithms by up to 7x over the A100 GPU. Two examples include the Smith-Waterman algorithm for genomics processing, and the Floyd-Warshall algorithm used to find optimal routes for a fleet of robots through a dynamic warehouse environment.

New thread block cluster feature enables programmatic control of locality at a granularity larger than a single thread block on a single SM. This extends the CUDA programming model by adding another level to the programming hierarchy to now include threads, thread blocks, thread block clusters, and grids. Clusters enable multiple thread blocks running concurrently across multiple SMs to synchronize and collaboratively fetch and exchange data.

Distributed shared memory allows direct SM-to-SM communications for loads, stores, and atomics across multiple SM shared memory blocks.

New asynchronous execution features include a new Tensor Memory Accelerator (TMA) unit that can transfer large blocks of data efficiently between global memory and shared memory. TMA also supports asynchronous copies between thread blocks in a cluster. There is also a new asynchronous transaction barrier for doing atomic data movement and synchronization.

New transformer engine uses a combination of software and custom Nvidia Hopper Tensor Core technology designed specifically to accelerate transformer model training and inference. The transformer engine intelligently manages and dynamically chooses between FP8 and 16-bit calculations, automatically handling re-casting and scaling between FP8 and 16-bit in each layer to deliver up to 9x faster AI training and up to 30x faster AI inference speedups on large language models compared to the prior generation A100.
